Dynamic Data-Race Detection through the Fine-Grained Lens

Data races are among the most common bugs in concurrency. The standard approach to data-race detection is via dynamic analyses, which work over executions of concurrent programs, instead of the program source code. The rich literature on the topic has created various notions of dynamic data races, which are known to be detected efficiently when certain parameters (e.g., number of threads) are small. However, the \emph{fine-grained} complexity of all these notions of races has remained elusive, making it impossible to characterize their trade-offs between precision and efficiency. In this work we establish several fine-grained separations between many popular notions of dynamic data races. The input is an execution trace with $N$ events, $T$ threads and $L$ locks. Our main results are as follows. First, we show that happens-before (HB) races can be detected in $O(N\cdot \min(T, L))$ time, improving over the standard $O(N\cdot T)$ bound when $L=o(T)$. Moreover, we show that even reporting an HB race that involves a read access is hard for 2-orthogonal vectors (2-OV). This is the first rigorous proof of the conjectured quadratic lower-bound in detecting HB races. Second, we show that the recently introduced synchronization-preserving races are hard to detect for OV-3 and thus have a cubic lower bound, when $T=\Omega(N)$. This establishes a complexity separation from HB races which are known to be less expressive. Third, we show that lock-cover races are hard for 2-OV, and thus have a quadratic lower-bound, even when $T=2$ and $L = \omega(\log N)$. The similar notion of lock-set races is known to be detectable in $O(N\cdot L)$ time, and thus we achieve a complexity separation between the two. Moreover, we show that lock-set races become hitting-set (HS)-hard when $L=\Theta(N)$, and thus also have a quadratic lower bound, when the input is sufficiently complex.

==> other.tex <==
\begin{theorem}
\thmlabel{cedl-to-ov-reduction}
The special case of \cedl{} where (i) the number of access events, say $\NumEvents_{acc}$ is much larger than the sum of distinct locks and threads, (ii) sum of locks and threads is $\omega(\log \NumEvents_{acc})$, and (iii) where all the access events are to a single memory location, fine-grained reduces to \orthv{}. 
\end{theorem}
\begin{proof}
Given a trace $\sigma$ of the special case of \cedl{}, we construct an instance \ovinstwo{} of \orthv{} as follows. The \orthv{} instance has the same set of vectors in both parts. Each access event of $\sigma$ corresponds to a vector in each part of \orthv{}, thus $n$ is the number of access events in $\sigma$. Let $l$ be the maximum number of locks held by any access event in $\sigma$, and $k$ be the number of distinct thread identifiers from all events. Then $d=l+k+1,$ and the vector $v$ corresponding to an event $e$ is defined as follows. The $i^{th}$ of the first $l$ coordinates of $v$ is $1$ only if the $i^{th}$ lock is held by the event. Among the next $k$ coordinates, only the one corresponding to the thread identifier of $e$ is $1$. Finally, the $(l+k+1)^{st}$ coordinate is $1$ if the event is a read access event, and $0$ otherwise. 

Let us see why this reduction is correct. Suppose $a$ and $b$ are orthogonal vectors and a solution to \orthv{}. Let $e_a$ and $e_b$ be their corresponding events in $\sigma.$ First, note that $e_a$ and $e_b$ cannot both be read events, as otherwise the last coordinates of $a$ and $b$ would be $1,$ contradicting their orthogonality. Next, $e_a$ and $e_b$ would belong in different threads, else the same coordinate corresponding to their common thread identifier would be $1$ in $a$ and $b,$ again contradicting orthogonality. Thus, $e_a$ and $e_b$ are conflicting events. Finally, as $a$ and $b$ are orthogonal, none of their first $l$ coordinates are both $1,$ implying that $e_a$ and $e_b$ do not hold a common lock. Hence, $\lheld{\tr}(e_a)\cap\lheld{\tr}(e_b)=\emptyset,$ hence $e_a,e_b$ is a solution to \cedl{}. A similar argument can show that a solution to the given \cedl{} instance would correspond to a solution of \orthv{}. 

Hence, in $O(\NumEvents)$ time, where $\NumEvents$ are the number of events in $\sigma,$ we have reduced the special case of \cedl{} to an instance of \orthv{} \ovinstwo{} where $n$ is the number of access events, say $\NumEvents_{acc},$ and $d=o(\log \NumEvents_{acc}).$ Hence, an $O(n^{(2-\epsilon)}\cdot \poly(d))$ time algorithm for \orthv{} implies an $O(\NumEvents_{acc}^{(2-\epsilon)}\cdot \poly(o(\NumEvents_{acc})))$ time algorithm, which is $O(\NumEvents^{(2-\epsilon')})$ for some $\epsilon'$, for the special case of \cedl{}.  
\end{proof}

==> summary.tex <==
%!TEX root = main.tex

\section{Summary of Results}

%\begin{restatable}{theorem}{cedl-quadratic-lower-bound}\thmlabel{cedl-quadratic-lower-bound}
%Assuming \ovc, the problem \cedl~cannot be solved in
%time $o(\NumEvents^2\NumLocks)$, where $\NumEvents$ is the number of \rcomment{access} events
%and $\NumLocks$ is the number of locks in the input trace.
%\end{restatable}

The algorithm of \cite{Savage97} processes the trace in
a one-pass streaming fashion and \rcomment{solves \nclv{}} in linear time, assuming parameters
like $\NumLocks$ are constant.
Is the assumption of these parameters being constant crucial in
establishing the linear time upper bound?
In other words, is it possible to get a linear time algorithm
if this assumption is relaxed? We show a conditional negative answer to the latter question, assuming \hsc{}. First we show why \ovc{} cannot be used to show such a result. Corollary $2$ from \cite{CarmosinoGIMPS2016} implies that if there is a non-deterministic linear time algorithm for a problem and its complement, that is, a linear time verifiable certificate for both positive and negative instances of the problem, then assuming \nseth{}, any conjecture that assumes \seth{} cannot be used to prove a higher than linear time lower bound. We show that such a \rcomment{linear time algorithm} exists for \nclv{}.

%\begin{restatable}{theorem}{nclv-no-seth-hardness}\thmlabel{nclv-no-seth-hardness}
%$\nclv{}\in \ntime{n}\cap \contime{n}.$ 
%\end{restatable}

%As a reduction from OV is not possible unless NSETH is false, we prove a hardness assuming the HS conjecture. 

The proof of \thmref{nclv-no-seth-hardness} implies an $O(\NumEvents\cdot \min\{\NumLocks,\NumVariables\})$ time algorithm. Contrast this with \thmref{cedl-quadratic-lower-bound}, which shows that \cedl{} is $\Omega(\NumEvents^2)$ hard even with $1$ memory location access and $O(\log\NumEvents)$ locks. We next show a conditional $\Omega(\NumEvents^2)$ hardness for \nclv{} assuming \hsc{}, matching its upper bound when there are $O(\NumEvents)$ number of locks and as many memory location accesses.

% In this paper we establish that, in fact, in general
% when this assumption is relaxed, the problem is conditionally hard.
% In particular, \ucomment{characterize the results of the following two theorems}.

%\begin{restatable}{theorem}{nclv-quadratic-lower-bound}\thmlabel{nclv-quadratic-lower-bound}
%Assuming \hsc{}, the problem \nclv{} cannot be solved in time $o(\NumEvents^2)$ where $\NumEvents$ is the number of \rcomment{access} events
%and there are $O(\NumEvents)$ number of locks and memory locations, i.e., $\NumLocks=O(\NumEvents)$ and $\NumVariables=O(\NumEvents)$.  
%\end{restatable}

We then turn our attention to detecting $\HB$-races dynamically.
As observed \ucomment{in sec..}, the popular vector clock algorithm for detecting
$\HB$-races runs in time 

\rcomment{Placeholder content from here till end of section.}

We first show an algorithm with an improved bound of $O(\NumEvents\min\{\NumThreads,\NumLocks\})$, then prove that the general problem is hard under \ovc.

%\begin{restatable}{theorem}{hb-algo}\thmlabel{hb-algo}
%\rcomment{hb-algo}
%\end{restatable}

%\begin{restatable}{theorem}{hb-ov-hard}\thmlabel{hb-ov-hard}
%\rcomment{hb-ov-hard}
%\end{restatable}

As listing all $\HB$-races is unlikely to have a sub-quadratic algorithm, it is then natural to ask if the problem of deciding whether a given trace has an $\HB$-race is easier. We show that this decision version too will not have a better than $O(\NumEvents^{3/2})$ time algorithm. We also show, using \thmref{better-than-t-unlikely-under-seth}, that a better lower bound under \seth{} is improbable. 

%\begin{restatable}{theorem}{hb-decide-mc-hard}\thmlabel{hb-decide-mc-hard}
%\rcomment{hb-decide-mc-hard}
%\end{restatable}

%\begin{restatable}{theorem}{hb-decide-no-seth-better-than-3/2}\thmlabel{hb-decide-no-seth-better-than-3/2}
%\rcomment{no seth better than 3/2}
%\end{restatable}

Finally we show that the problem of detecting sync preserving races is even harder, by giving a cubic lower bound under \ovc{} for the same. We show this bound is tight in the sense that a better bound cannot be obtained conditioned on \seth{}.

%\begin{restatable}{theorem}{syncp-ov3-hard}\thmlabel{syncp-ov3-hard}
%\rcomment{syncp ov 3 hard}
%\end{restatable}

%\begin{restatable}{theorem}{syncp-no-seth-better-than-3}\thmlabel{syncp-no-seth-better-than-3}
%\rcomment{syncp no seth better than 3}
%\end{restatable}

